PlaneSLAM: Plane-based LiDAR SLAM for Motion Planning in Structured 3D Environments

LiDAR sensors are a powerful tool for robot simultaneous localization and mapping (SLAM) in unknown environments, but the raw point clouds they produce are dense, computationally expensive to store, and unsuited for direct use by downstream autonomy tasks, such as motion planning. For integration with motion planning, it is desirable for SLAM pipelines to generate lightweight geometric map representations. Such representations are also particularly well-suited for man-made environments, which can often be viewed as a so-called "Manhattan world" built on a Cartesian grid. In this work we present a 3D LiDAR SLAM algorithm for Manhattan world environments which extracts planar features from point clouds to achieve lightweight, real-time localization and mapping. Our approach generates plane-based maps which occupy significantly less memory than their point cloud equivalents, and are suited towards fast collision checking for motion planning. By leveraging the Manhattan world assumption, we target extraction of orthogonal planes to generate maps which are more structured and organized than those of existing plane-based LiDAR SLAM approaches. We demonstrate our approach in the high-fidelity AirSim simulator and in real-world experiments with a ground rover equipped with a Velodyne LiDAR. For both cases, we are able to generate high quality maps and trajectory estimates at a rate matching the sensor rate of 10 Hz.

==> sections/outline.tex <==
\section*{Outline}
\begin{outline}[enumerate]
    \1 Abstract (0.25 pg)
    \1 Introduction (0.5 pg)
        \2 SLAM is a key functionality for any robot operating in an unknown environment
            \3 Localization is necessary for navigation, mapping is necessary for collision avoidance, higher-level understanding, can also be desired final output for many applications
        \2 LiDAR has emerged as a powerful sensor for spatial mapping/SLAM
            \3 Vision methods have shown impressive results, however camera-based methods must rely on depth estimation rather than having reliable sensor-based depth information. Also vision fails in certain conditions such as low light
        \2 LiDAR naturally returns a point cloud, which is a dense representation of the environment
            \3 Point clouds take up large amounts of memory, also can be expensive to compute on for registration, etc.
            \3 Points which lie on the same plane or surface can often be represented together with a single object which uses much less memory and computationally cheaper to work with
        \2 We present an approach for LiDAR localization and mapping which extracts plane features from point clouds for registration and map creation 
            \3 Speeds up registration
            \3 Produces planar maps which take up much less memory and also lend themselves naturally to trajectory planning and collision avoidance.
    \1 Related work (0.75 pg)
        \2 LiDAR SLAM
            \3 Most state-of-the-art LiDAR SLAM methods still generate point cloud maps
            \3 LOAM \cite{zhang2014loam} - first demonstration of real-time LiDAR odometry and mapping
                \4 Extensions to LOAM: A-LOAM, F-LOAM \cite{wang2021f}, improves on localization accuracy and compute time (500 ms down to 200 ms/100 ms)
            \3 These point cloud maps grow rapidly in memory size as robot operation goes on and more area is explored \red{(do they grow in size even when the robot is sitting still? more points added as higher resolution)}
        \2 Plane methods
            \3 Extracting planes from point clouds itself is not a new idea
                \4 \cite{yang2010plane} proposes using RANSAC and minimum description length (MDL) for plane detection in point cloud data.
                \4 Region growing \cite{vo2015octree}
                \4 \cite{castagno2020polylidar3d} presents a fast non-convex polygon extraction algorithm that uses triangulation to create a mesh then segments planes and extracts polygons
                \4 Our work builds on these methods and leverages them for the frontend (feature extraction) of the SLAM problem
            \3 \cite{pathak2010online} demonstrates plane-based registration and SLAM in two real-world disaster scenarios which generates surface-based maps that are orders of magnitude smaller than their point cloud equivalents (avg 3.235 MB vs 124 kB). However, their approach of using arbitrary shaped surfaces leads to a visually more cluttered map that is also less conducive to path planning and other tasks. 
            \3 \cite{grant2019efficient} presents a LiDAR SLAM approach which exploits the structure of planar environments when available, using both point and plane features. \red{add in difference of our work: focuses more on connected consistent map output?}
            \3 \cite{favre2021plane} examines plane-based registration of LiDAR point clouds in detail, but does not consider the topic of SLAM and map creation
            
        % \2 Implicit representation methods
        % (Kimera uses visual inertial sensing to get fast good results metric semantic mesh)
        % (Inspired by Wireframe mapping?)
    \1 Problem statement (<0.25 pg)
        \2 Given a robot equipped with LiDAR sensor traveling through an unknown environment, our goal is to accurately estimate its motion while simultaneously constructing a sparse planar map of the environment.
            \3 
            \3 Key requirement is to build the sparse map in real-time, so that it can be used online for trajectory planning and other downstream autonomy tasks
    \1 Approach (2 pg)
        \2 Plane extraction
            \3 Algorithm block
            \3 Meshing
                \4 Spherical mapping
                \4 (scipy) Delaunay triangulation
                \4 Pruning
            \3 Clustering
                \3 Graph search
            \3 Extraction
        \2 Plane registration
            \3 
        \2 Mapping
            \3 Scan merging
            
    \1 Results (2 pg)
        \2 Metrics: 
            \3 Trajectory rotational/translational error
            \3 Comparison of frontend to PCL region growing
                \4 Comparable speed, better quality (less disjoint planes, etc)
        \2 Figures:
            \3 Final maps, trajectories
        \2 Simulation (AirSim)
        \2 Real-world (Rover)
    
        
\end{outline}
